Meta-learning enhanced next POI recommendation by leveraging check-ins from auxiliary cities

Most existing point-of-interest (POI) recommenders aim to capture user preference by employing city-level user historical check-ins, thus facilitating users' exploration of the city. However, the scarcity of city-level user check-ins brings a significant challenge to user preference learning. Although prior studies attempt to mitigate this challenge by exploiting various context information, e.g., spatio-temporal information, they ignore to transfer the knowledge (i.e., common behavioral pattern) from other relevant cities (i.e., auxiliary cities). In this paper, we investigate the effect of knowledge distilled from auxiliary cities and thus propose a novel Meta-learning Enhanced next POI Recommendation framework (MERec). The MERec leverages the correlation of check-in behaviors among various cities into the meta-learning paradigm to help infer user preference in the target city, by holding the principle of "paying more attention to more correlated knowledge". Particularly, a city-level correlation strategy is devised to attentively capture common patterns among cities, so as to transfer more relevant knowledge from more correlated cities. Extensive experiments verify the superiority of the proposed MERec against state-of-the-art algorithms.

==> tables/comparative.tex <==
\begin{table*}[t]
\centering
\footnotesize
\addtolength{\tabcolsep}{-2.2pt}
\caption{Comparative results of all approaches on the four datasets, where `H' refers to `Hit Ratio' and `N' means `NDCG'; the best results are highlighted in bold and the runner up is underlined; the column `Improve' indicates the improvements achieved by MERec relative to the runner up.}\label{tab2}
\begin{tabular}{cl|cc|ccc|ccc|r}
\toprule
& & \multicolumn{2}{c|}{\textbf{TM}} 
& \multicolumn{3}{c|}{\textbf{DL}}     
& \multicolumn{3}{c|}{\textbf{META}}
& \multirow{2}{*}{\textit{Improve}} \\
&  & MostPop & BPRMF & NeuMF  & ASTA-LSTM & iMTL   & MAML & CHAML   & MERec &  \\ \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Calgary}}}   
&{H@5}  & 0.0988          & 0.1304         & 0.1431 & 0.2924    & 0.2652 & 0.3987  & \underline{0.3995} & \textbf{0.4274} & 6.98\%                            \\
%%%%%%
&{H@10} & 0.1547          & 0.2349         & 0.2368 & 0.3705    & 0.3184 & 0.4618       & \underline{0.4777} & \textbf{0.5054} & 5.80\%                            \\
%%%%%%%
& {N@5}  & 0.0632          & 0.0928         & 0.0989 & 0.2134    & 0.1857 & \underline{0.3178} & 0.3093       & \textbf{0.3378} & 6.29\%                            \\
%%%%%%%%
&{N@10} & 0.0814          & 0.1672         & 0.1669 & 0.2383    & 0.2299 & \underline{0.3362} & 0.3315       & \textbf{0.3564} & 6.01\% \\ \hline
%%%%%%%%%
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Phoenix}}}   &{H@5}  & 0.0682          & 0.1093         & 0.1316 & 0.2366    & 0.2410 & 0.3549       & \underline{0.3660} & \textbf{0.3928} & 7.32\%                            \\
%%%%%%%%%
&{H@10} & 0.1068          & 0.1584         & 0.1852 & 0.3125    & 0.3370 & \underline{0.4508} & 0.4419       & \textbf{0.4531} & 0.51\%                            \\
%%%%%%%
& {N@5}  & 0.0419          & 0.0688         & 0.0869 & 0.1635    & 0.1753 & 0.2633       & \underline{0.2648} & \textbf{0.2796} & 5.59\%                            \\
%%%%%%%%%
& \multicolumn{1}{c|}{N@10} & 0.0547          & 0.0848         & 0.1042 & 0.1883    & 0.2065 & \underline{0.2949} & 0.2891       & \textbf{0.2993} & 1.49\%                            \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Singapore}}} & \multicolumn{1}{c|}{H@5}  & 0.0365          & 0.0848         & 0.1004 & 0.2165    & 0.2388 & 0.2991       & \underline{0.3571} & \textbf{0.3705} & 3.74\%  \\
& \multicolumn{1}{c|}{H@10} & 0.0635          & 0.1450         & 0.1696 & 0.2879    & 0.3080 & 0.3816       & \underline{0.4486} & \textbf{0.4488} & 0.04\%                            \\
                           & \multicolumn{1}{c|}{N@5}  & 0.0231          & 0.0452         & 0.0697 & 0.1532    & 0.1696 & 0.2188       & \underline{0.2650} & \textbf{0.2707} & 2.15\%                            \\
                           & \multicolumn{1}{c|}{N@10} & 0.0318          & 0.0648         & 0.0925 & 0.1760    & 0.1922 & 0.2451       & \underline{0.2981} & \textbf{0.2998} & 0.57\%                            \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{New York}}}  & \multicolumn{1}{c|}{H@5}  & 0.0214          & 0.0558         & 0.0959 & 0.1763    & 0.2187 & 0.2456     &\underline{0.2745} & \textbf{0.2991} & 8.96\%                            \\
                           & \multicolumn{1}{c|}{H@10} & 0.0336          & 0.0994         & 0.1495 & 0.2455    & 0.2879 & 0.3373       & \underline{0.3526} & \textbf{0.3995} & 13.3\%                            \\
                           & \multicolumn{1}{c|}{N@5}  & 0.0134          & 0.0265         & 0.0595 & 0.1257    & 0.1484 & 0.1652       & \underline{0.1865} & \textbf{0.2107} & 12.98\%                           \\
                           & \multicolumn{1}{c|}{N@10} & 0.0173          & 0.0237         & 0.0770 & 0.1485    & 0.1705 & 0.2072       & \underline{0.2118} & \textbf{0.2436} & 15.01\%                           \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/table_results__10.tex <==
\begin{table*}[t]
	\centering
	\scriptsize
	\caption{Comparison results on the four datasets w.r.t HR@10 and NDCG@10.}
        %\textcolor{red}{add results}
	%\vspace{-0.15in}
	%\addtolength{\tabcolsep}{-0.4pt}
	%\addtolength{\tabcolsep}{1.7pt}
	\renewcommand{\arraystretch}{1.3} % Default value: 1
	\begin{tabular}{c|c|cc|cc|cc|cc} 
	\specialrule{.15em}{.05em}{.05em}
         \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{CAL} & \multicolumn{2}{c|}{PHO}& \multicolumn{2}{c|}{SIN} & \multicolumn{2}{c}{NYC}\\
		\cline{3-10}
		\multicolumn{2}{c|}{}  & HR@10 & NDCG@10 & HR@10 & NDCG@10 & HR@10 & NDCG@10 & HR@10 & NDCG@10\\
		\specialrule{.05em}{.05em}{.05em}
        \multirow{2}{*}{TM} & MostPop & 0.1547  & 0.0814 & 0.1068 & 0.0547 & 0.0635  & 0.0318 & 0.0336 & 0.0173\\
        & BPRMF & 0.2349  & 0.1672 & 0.1584 & 0.0848 & 0.1450  & 0.0648 & 0.0994 & 0.0237\\
        \hline
        \multirow{3}{*}{DL} & NeuMF & 0.2368  & 0.1669 & 0.1852 & 0.1042 & 0.1696  & 0.0925 & 0.1495 & 0.0770\\
        & ATST-LSTM & 0.3705  & 0.2384 & 0.3125 & 0.1883 & 0.2879  & 0.1760 & 0.2455 & 0.1485\\
        & iMTL & 0.3184  & 0.2299 & 0.3370 & 0.2065 & 0.3080  & 0.1922 & 0.2879 & 0.1705\\
        \hline
        \multirow{3}{*}{META} & MAML & 0.4618  & \underline{0.3362} & \underline{0.4508} & \underline{0.2949} & 0.3816  & 0.2451 & 0.3373 & 0.2072\\
        & CHAML & \underline{0.4777}  & 0.3315 & 0.4419 & 0.2891 & \underline{0.4486}  & \underline{0.2981} & \underline{0.3526} & \underline{0.2118}\\
        & MERec &  \textbf{0.5054}  & \textbf{0.3564} & \textbf{0.4531} & \textbf{0.2993} & \textbf{0.4488}  & \textbf{0.2998} & \textbf{0.3995} & \textbf{0.2436}\\
        \hline
        \multicolumn{2}{c|}{Improvement} & 5.80\% & 6.01\%& 0.51\%& 1.49\%& 0.04\% & 0.57\%& 13.3\%&15.01\%\\
		\specialrule{.15em}{.05em}{.05em}
	\end{tabular}
	\label{table:comparison_results_10}
	\vspace{-0.1in}
\end{table*}






==> tables/table_results__5.tex <==
\begin{table*}[t]
	\centering
	\scriptsize
	\caption{Comparison results on the four datasets w.r.t HR@5 and NDCG@5.}
        %\textcolor{red}{add results}
	%\vspace{-0.15in}
	%\addtolength{\tabcolsep}{-0.4pt}
	%\addtolength{\tabcolsep}{1.7pt}
	\renewcommand{\arraystretch}{1.2} % Default value: 1
	\begin{tabular}{c|c|cc|cc|cc|cc} 
	\specialrule{.15em}{.05em}{.05em}
         \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{CAL} & \multicolumn{2}{c|}{PHO}& \multicolumn{2}{c|}{SIN} & \multicolumn{2}{c}{NYC}\\
		\cline{3-10}
		\multicolumn{2}{c|}{}  & HR@10 & NDCG@10 & HR@10 & NDCG@10 & HR@10 & NDCG@10 & HR@10 & NDCG@10\\
		\specialrule{.05em}{.05em}{.05em}
        \multirow{2}{*}{TM} & MostPop & 0.0988  & 0.0632 & 0.0682 & 0.0419 & 0.0365  & 0.0231 & 0.0214 & 0.0134\\
        & BPRMF & 0.1304  & 0.0928 & 0.1093 & 0.0688 & 0.0848  & 0.0452 & 0.0558 & 0.0265\\
        \hline
        \multirow{3}{*}{DL} & NeuMF & 0.1431  & 0.0989 & 0.1316 & 0.0869 & 0.1004  & 0.0697 & 0.0959 & 0.0595\\
        & ATST-LSTM & 0.2924  & 0.2134 & 0.2366 & 0.1635 & 0.2165  & 0.1532 & 0.1763 & 0.1257\\
        & iMTL & 0.2652  & 0.1857 & 0.2410 & 0.1753 & 0.2388  & 0.1696 & 0.2187 & 0.1484\\
        \hline
        \multirow{3}{*}{META} & MAML & 0.3987  & \underline{0.3178} & 0.3549
        & 0.2633 & 0.2991  & 0.2188 & 0.2456 & 0.1652\\
        & CHAML & \underline{0.3995}  & 0.3093 & \underline{0.3660} & \underline{0.2648} & \underline{0.3571}  & \underline{0.2650} & \underline{0.2745} & \underline{0.1865}\\
        & MERec &  \textbf{0.4274}  & \textbf{0.3378} & \textbf{0.3928} & \textbf{0.2796} & \textbf{0.3705}  & \textbf{0.2707} & \textbf{0.2991} & \textbf{0.2107}\\
        \hline
        \multicolumn{2}{c|}{Improvement} & 6.98\% & 6.29\%& 7.32\%& 5.59\%& 3.74\% & 2.15\%& 8.96\%&12.98\%\\
		\specialrule{.15em}{.05em}{.05em}
	\end{tabular}
	\label{table:comparison_results_5}
	\vspace{-0.1in}
\end{table*}





